Intent-calibrated Self-training for Answer Selection in Open-domain Dialogues

Answer selection in open-domain dialogues aims to select an accurate answer from candidates. Recent success of answer selection models hinges on training with large amounts of labeled data. However, collecting large-scale labeled data is labor-intensive and time-consuming. In this paper, we introduce the predicted intent labels to calibrate answer labels in a self-training paradigm. Specifically, we propose the intent-calibrated self-training (ICAST) to improve the quality of pseudo answer labels through the intent-calibrated answer selection paradigm, in which we employ pseudo intent labels to help improve pseudo answer labels. We carry out extensive experiments on two benchmark datasets with open-domain dialogues. The experimental results show that ICAST outperforms baselines consistently with 1%, 5% and 10% labeled data. Specifically, it improves 2.06% and 1.00% of F1 score on the two datasets, compared with the strongest baseline with only 5% labeled data.

==> contents/taclformat.tex <==
\iftaclpubformat

\onecolumn


Option 1. Author’s address is underneath each name, centered.

\begin{quote}\centering
  \begin{tabular}{c}
    \textbf{First Author} \\
    First Affiliation \\
    First Address 1 \\
    First Address 2 \\
    \texttt{first.email@example.com}
  \end{tabular}
  \ 
  \begin{tabular}{c}
    \textbf{Second Author} \\
    Second Affiliation \\
    Second Address 1 \\
    Second Address 2 \\
    \texttt{second.email@example.com}
  \end{tabular}

  \begin{tabular}{c}
    \textbf{Third Author} \\
    Third Affiliation \\
    Third Address 1 \\
    Third Address 2 \\
    \texttt{third.email@example.com}
  \end{tabular}
\end{quote}
  

Option 2. Author’s address is linked with superscript characters to its name,
author names are grouped, centered.

\begin{quote}\centering
    \textbf{First Author$^\diamond$} \quad \textbf{Second Author$^\dagger$} \quad
    \textbf{Third Author$^\ddagger$}
    \\ \ \\
    $^\diamond$First Affiliation \\
    First Address 1 \\
    First Address 2 \\
    \texttt{first.email@example.com}
     \\ \ \\
     $^\dagger$Second Affiliation \\
    Second Address 1 \\
    Second Address 2 \\
    \texttt{second.email@example.com}
     \\ \ \\
    $^\ddagger$Third Affiliation \\
    Third Address 1 \\
    Third Address 2 \\
    \texttt{third.email@example.com}
\end{quote}
  
\fi
